$\Delta$-Machine Learning for Potential Energy Surfaces: A PIP approach to bring a DFT-based PES to CCSD(T) Level of Theory

``$\Delta$-machine learning" refers to a machine learning approach to bring a property such as a potential energy surface (PES) based on low-level (LL) density functional theory (DFT) energies and gradients to close to a coupled cluster (CC) level of accuracy. Here we present such an approach that uses the permutationally invariant polynomial (PIP) method to fit high-dimensional PESs. The approach is represented by a simple equation, in obvious notation $V_{LL{\rightarrow}CC}=V_{LL}+\Delta{V_{CC-LL}}$, and demonstrated for \ce{CH4}, \ce{H3O+}, and $trans$ and $cis$-$N$-methyl acetamide (NMA), \ce{CH3CONHCH3}. For these molecules, the LL PES, $V_{LL}$, is a PIP fit to DFT/B3LYP/6-31+G(d) energies and gradients, and $\Delta{V_{CC-LL}}$ is a precise PIP fit obtained using a low-order PIP basis set and based on a relatively small number of CCSD(T) energies. For \ce{CH4} these are new calculations adopting an aug-cc-pVDZ basis, for \ce{H3O+} previous CCSD(T)-F12/aug-cc-pVQZ energies are used, while for NMA new CCSD(T)-F12/aug-cc-pVDZ calculations are performed. With as few as 200 CCSD(T) energies, the new PESs are in excellent agreement with benchmark CCSD(T) results for the small molecules, and for 12-atom NMA training is done with 4696 CCSD(T) energies.

==> ch4.tex <==
\subsection{\ce{CH4}}
For the present work we use one of the recent DFT/B3LYP-based PESs for methane, as noted above.\cite{NandiQuBowman2019} This PES was developed to demonstrate new PIP software for fitting energies and gradients.\cite{msachen} This PES is based on precise fitting energies and gradients at 600 configurations.  Here, this PES is brought to the CCSD(T) level of accuracy.   

We trained $\Delta{V_{CC-LL}}$ using the difference of CCSD(T) and DFT absolute energies and then test on a different set. A variety of training datasets were used and details of one example are shown in In Fig. \ref{fig:Corr_ch4}. There we plot  $\Delta{V_{CC-LL}}$ versus the DFT energies for a training set of 600 configurations.  Testing the fit is done on a larger dataset of 2000  energy differences, shown in the lower panel of this figure.  For clarity we reference $\Delta{V_{CC-LL}}$ to the minimum of the  difference of the CCSD(T) and DFT energies (which is roughly -19 820 cm$^{-1}$). As seen, the energy range of $\Delta{V_{CC-LL}}$ is about 1600 cm$^{-1}$, which is much smaller than the DFT energy range relative to the minimum value (which is roughly 15 000 cm$^{-1}$). Also note the training dataset looks like a ``thinned" version of the larger test dataset. 


\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.9\columnwidth]{Delta-train-test.pdf}
    \caption{Plot of $\Delta{V_{CC-LL}}$ (relative to the reference value i.e. -19 820 cm$^{-1}$) vs DFT energy relative to the \ce{CH4} minimum value with the indicated number of training and test data set.}
    \label{fig:Corr_ch4}
\end{figure}

 $\Delta{V_{CC-LL}}$ was fit using a dataset of 600 energies using a PIP (describing the 4! permutations of the H atoms) basis with maximum polynomial order 5. This results in a basis of 208 terms. The linear coefficients were determined by solving the  linear least-squares problem; the fitting RMS error of this $\Delta{V_{CC-LL}}$ fit is 0.18 cm$^{-1}$. The fit was tested on the 2000 energy differences. The RMS test error in this case is 0.79 cm$^{-1}$.

To obtain the corrected PES $V_{LL{\rightarrow}CC}$ we add $\Delta{V_{CC-LL}}$ to one of our previously reported DFT-based PESs for \ce{CH4}.\cite{NandiQuBowman2019} The fitting RMS error of that $V_{LL}$ DFT PES is 2.55 cm$^{-1}$. To examine how well the corrected PES $V_{LL{\rightarrow}CC}$ reproduces the CCSD(T) energies we plot the energies of $V_{LL{\rightarrow}CC}$ vs the direct CCSD(T) energies for both training and test data sets in Fig. \ref{fig:fitting_ch4}. As seen, the correspondence between the two is excellent. The overall RMS differences are 2.5 and 3.2 cm$^{-1}$ for the training and testing set, respectively. This is already an indication of the success of the present approach to correct the DFT-based PES and bring the corrected PES very close to CCSD(T) energies. 


To examine the robustness of these results, fits of $\Delta{V_{CC-LL}}$ were also done using  datasets of 1000, 300, and 100 energies. The corresponding RMS differences between the $V_{LL{\rightarrow}CC}$ and CCSD(T) energies are given in Table \ref{tab:tab_ch4}. In case of the training set with $N_{Train} = 1000$, we use a maximum polynomial order of 5 to fit $\Delta{V_{CC-LL}}$, and this leads to a basis of 208 terms. For the training data set of 300 and 100, we reduce the maximum polynomial order to avoid overfitting. As seen, the RMS errors are similar for all the training data sets. This is certainly notable for the training set of only 100 energy differences, where the RMS error is only 4.9 cm$^{-1}$ for the 2000 test energies up to 15000 cm$^{-1}$. In this case the PIP basis for  $\Delta{V_{CC-LL}}$ contains only 30 terms.  

Next consider the performance of the $\Delta$-ML approach  for the equilibrium geometry and normal mode frequencies.  The results are compared to the CCSD(T) and DFT ones in Table \ref{tab:tab_ch4_2}. As seen, the corrected PES $V_{LL{\rightarrow}CC}$ produces results in excellent agreement with direct CCSD(T) ones and also provides a large improvement compared to the DFT PES. Perhaps most impressive is the high accuracy achieved even with the smallest training dataset of 100 energies.  


\begin{figure}[htbp!]
    \centering
    \includegraphics[width=1.0\columnwidth]{Methane-Fit-train-test.pdf}
    \caption{Plot of fitting errors with the indicated number of training and test data set for \ce{CH4}. Energies are relative to that of the global minimum. The upper panel represents the plot of fitting energy vs direct CCSD(T) energy and the lower panel represents the the fitting error at each energy.} 
    \label{fig:fitting_ch4}
\end{figure}

\begin{table}[htbp!]
\centering
\caption{RMS fitting error of energies (RMS$_{\rm E}$) (cm$^{-1}$) with the indicated number of training ($N_{\rm Train}$) and test ($N_{\rm Test}$) configurations for the \ce{CH4} molecule.}
\label{tab:tab_ch4}

\begin{threeparttable}
	\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}rrrr}
	\hline
	\hline\noalign{\smallskip}
%	  & \multicolumn{2}{c}{PES-E \tnote{a}} & \multicolumn{2}{c}{PES-EG} \\
%    \noalign{\smallskip} \cline{2-3} \cline{4-5} \noalign{\smallskip}
     $N_{\rm Train}$ & RMS$_{\rm E}$ & $N_{\rm Test}$ & RMS$_{\rm E}$ \\
	\noalign{\smallskip}\hline\noalign{\smallskip}
     1000\tnote{a} & 2.97 & 2000 & 3.14 \\
     600\tnote{a}  & 2.54 & 2000 & 3.22 \\
     300\tnote{b}  & 2.79 & 2000 & 4.41 \\
     100\tnote{c}  & 2.71 & 2000 & 4.88 \\
 
	\noalign{\smallskip}\hline
	\hline
   
	\end{tabular*}

   	\begin{tablenotes}
    \item[a] Maximum polynomial order of 5, basis size of 208.
    \item[b] Maximum polynomial order of 4, basis size of 83.
    \item[c] Maximum polynomial order of 3, basis size of 30.
    \end{tablenotes}
    
\end{threeparttable}   
\end{table}


\begin{table}[htbp!]
\centering
\caption{Comparison of differences, $\delta$, in bond lengths (angstroms) and harmonic frequencies (cm$^{-1}$) relative to direct CCSD(T) benchmarks for the minimum of \ce{CH4}. Note 2.0(-5) means $2.0 \times 10^{-5}$, etc }
\label{tab:tab_ch4_2}

\begin{threeparttable}
	\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}rrrrrrr}
	\hline
	\hline\noalign{\smallskip}
	  & \multicolumn{2}{c}{Geom. Param.} & \multicolumn{4}{c}{Harmonic Freq.} \\
    \noalign{\smallskip} \cline{2-3} \cline{4-7} \noalign{\smallskip}
     $N_{\rm Train}$ & $\delta$(C-H) & $\delta$(H-H) & $\delta$$v_{1}$ & $\delta$$v_{2}$ & $\delta$$v_{3}$& $\delta$$v_{4}$ \\
	\noalign{\smallskip}\hline\noalign{\smallskip}
     1000\tnote{a} & -2.0(-5) & -2.5(-5) & -0.9 & 1.8 & -1.1 & 0.5 \\
     600\tnote{a}  & -2.0(-5) & -2.5(-5) & -1.2 & 1.7 & -1.3 & 0.6 \\
     300\tnote{b}  & -3.0(-5) & -4.5(-5) & -0.2 & 1.7 & -0.1 & -0.1 \\
     100\tnote{c}  & -2.0(-5) & -3.5(-5) & -0.2 & 1.5 & -2.5 & 0.3 \\
	\noalign{\smallskip}\hline\noalign{\smallskip}
     DFT   & 8.1(-3) & 1.3(-2) & -46.1 & -47.2 & -25.32 & -4.0 \\ 
	\noalign{\smallskip}\hline
	\hline
   
	\end{tabular*}

   	\begin{tablenotes}
    \item[a] Maximum polynomial order of 5, basis size of 208.
    \item[b] Maximum polynomial order of 4, basis size of 83.
    \item[c] Maximum polynomial order of 3, basis size of 30.
    \end{tablenotes}	
\end{threeparttable}

\end{table}


%\begin{figure}[htbp!]
%    \centering
%    \includegraphics[width=1.0\columnwidth]{Hist-train-test.pdf}
%    \caption{Distribution of energies (cm$^{-1}$) relative to the minimum value of \ce{CH4} for both CCSD(T) and DFT training and test data sets.}
%    \label{fig:Histo_ch4}
%\end{figure}

%\begin{figure}[htbp!]
%   \centering
%    \includegraphics[width=1.0\columnwidth]{Delta-train-test.pdf}
%    \caption{Distribution of $\Delta$E (cm$^{-1}$) relative to the \ce{CH4} minimum value.}
%    \label{fig:Delta_ch4}
%\end{figure}
